Results from Particle-Resolved Simulations

We review some of the results obtained to date with the aid of the PR-DNS approach to turbulent particulate flows. It is shown that the method has matured to a point which allows to apply it successfully to a wide variety of fluid/particle configurations, albeit still at a relatively large computational cost. Due to the availability of high-fidelity space-and-time-resolved data, a number of challenging open questions have already been addressed in unprecedented detail.

==> FIG_AC/Visus_top_columns.tex <==
\begin{figure}
%
\begin{minipage}{0.475\linewidth}
    \centering{(a)}
	\begin{overpic}[width=1.\linewidth]
		{./FIG_AC/visu_uhlmann14.png}
		\put(-5.5,40){\rotatebox{90}{$y/d$}}
		\put(42.50,-5.5){$x/d$}
	\end{overpic}
\end{minipage}
%
\begin{minipage}{0.475\linewidth}
	\centering{(b)}
	\begin{overpic}[width=1.005\linewidth]
		{./FIG_AC/Visu_Huisman16.png}
	\end{overpic}
\end{minipage}
%
\caption{Top views of particle positions taken from the work of
  \citet{uhlmann:14a} (a) and \citet{huisman:16} (b). On (a) particles
  are colored according to the fluctuation of their vertical velocity
  scaled by the particle and time-averaged settling velocity, on (b)
  particles are colored according to their settling velocity. The
  polygons on (b) represent the borders of the Vorono\"i areas
  computed once all particle positions are projected on an horizontal
  plane.} 
\label{fig:PRS-2D_visus_columns}
\end{figure}

==> FIG_AC/settling_velocity_ambient.tex <==
\begin{figure}
   \begin{minipage}{0.5\linewidth}
      \centering
      \mbox{}\\[1.75cm]
      \begin{overpic}[width=0.9\linewidth]
         {./FIG_AC/SettlingVelocity_Phi.pdf}
         \put(-5,35){\rotatebox{90}{$\proofedit{w_{rel}}{W_{rel}}/W_{s}$}}
         \put(45,-5){$\phi$}
         % -------------------------------------------------------
         \put(45,80){(a)}
         % -------------------------------------------------------
         \put(-6,108)
             {\small \ACcircfull\, $\phi=0.01$, $\revision{Ga}{\mathrm{Ga}}=145$ \cite{fornari:18a}}
         \put(-6,102)
             {\small \ACdiamond\, $\phi=0.05$, $19 \leq \revision{Ga}{\mathrm{Ga}} \leq 200$ \cite{fornari:16d}}
             %% \cite{fornari:16c} %% PROOF
         \put(-6,96)
            {\small \ACtrileft\, oblate spheroids }
         \put(-3,91)
            {\small (aspect ratio 1/3), $\revision{Ga}{\mathrm{Ga}}=60$ \cite{fornari:18b}}
         \put(-6,85)
            {\small \textcolor{ACred}{\ACtriup} $\revision{Re_{ps}}{\mathrm{Re_{ps}}} < 10^{-3}$ \cite{nicolai:95}}
         % -------
         \put(152,108)
             {\small \textcolor{ACblue}{\ACcirc} spheres,
                          \textcolor{ACblue}{\ACsquare} cubes,
                           $\revision{Ga}{\mathrm{Ga}}=160$ \cite{seyed:21}}
         \put(152,102)
             {\small \textcolor{ACdarkblue}{\ACcirc} spheres,
                          \textcolor{ACdarkblue}{\ACsquare} cubes,
                           $\revision{Ga}{\mathrm{Ga}}=70$ \cite{seyed:21}}
         \put(152,96)
             {\small \textcolor{blue}{\ACtridown} $2\times 10^{-4} \leq \phi \leq 0.001$,}
         \put(154,91){ \small   $110 \leq \revision{Ga}{\mathrm{Ga}} \leq 310$ 
                          \cite{huisman:16}}
         % -------
         \put(60,108)
             {\small  \textcolor{ACgreen}{\ACdiamond} $\phi=0.005$, $\revision{Ga}{\mathrm{Ga}}=121$,
                          \textcolor{ACgreen}{\ACcirc} $\revision{Ga}{\mathrm{Ga}}=178$,
                          \cite{uhlmann:14a}}
         \put(60,102)
            {\small  \textcolor{ACgreen}{\ACcircfull} $\phi=0.0005$, $\revision{Ga}{\mathrm{Ga}}=178$,
                         \cite{todor_phd}}
         \put(60,96)
             {\small \textcolor{ACyellow}{\ACcross} $\phi=0.003$, 
                     \textcolor{ACyellow}{\ACcirc}\, $\phi=0.01$, $0.1 \leq \revision{Re_{ps}}{\mathrm{Re_{ps}}} \leq 10$ \cite{climent:03}}
         \put(60,90)
             {\small \textcolor{ACpurple}{\ACcross} $\phi=0.003$, 
                     \textcolor{ACpurple}{\ACcirc}\, $\phi=0.01$, $1 \leq \revision{Re_{ps}}{\mathrm{Re_{ps}}} \leq 300$ \cite{zaidi:14}}
      \end{overpic}
   \end{minipage}
   %
   \begin{minipage}{0.5\linewidth}
      \centering
      \mbox{}\\[1.75cm]
      \begin{overpic}[width=0.9\linewidth]
         {./FIG_AC/SettlingVelocity_Ga.pdf}
         \put(45,-5){$\revision{Ga}{\mathrm{Ga}}$}
         % -------------------------------------------------------
         \put(45,80){(b)}
         % -------------------------------------------------------
      \end{overpic}
   \end{minipage}
   \mbox{}\\[-0.2cm]
   \caption{Evolution of the mean particle settling velocity
     $W\revision{}{_z}$ scaled by the corresponding single-sphere
     value $W_s$ for different simulations and experiments in ambient
     fluid represented as a function of the solid volume fraction (a)
     and Galileo number (b). When not mentioned in the legend, the
     data refers to spherical particles. \revision{}{Colorstyle is
       common for (a) and (b), data from references \cite{climent:03}
       and \cite{zaidi:14} are represented exclusively with crosses on
       (a).}} 
   \label{fig:PRS-settling_vel_ambient}
\end{figure}
